Aerodynamic Characterization of a Fan Array Wind Generator

Experimental assessment of safe and precise flight control algorithms for unmanned aerial vehicles (UAVs) under gusty wind conditions requires the capability to generate a large range of velocity profiles. In this study, we employ a small fan array wind generator which can generate flows with large spatial and temporal variability. We perform a thorough aerodynamic characterization operating the fans uniformly from a low to the maximum level. PIV and hot-wire measurements indicate a jet-like flow with nearly uniform core which monotonously contracts in streamwise direction and surrounding growing unsteady shear-layers. These complex dynamics results in a limited region with desired flow profile and turbulence level. The experimental results shed light on the flow generated by a full-scale fan array wind generator, and indicate the need for further improvements via properly designed add-ons and dedicated control algorithms.

==> nomenclature.tex <==
\section*{Nomenclature}

\noindent(Nomenclature entries should have the units identified)

{\renewcommand\arraystretch{1.0}
	\noindent\begin{longtable*}{@{}l @{\quad=\quad} l@{}}
		$A$  & amplitude of oscillation \\
		$a$ &    cylinder diameter \\
		$C_p$& pressure coefficient \\
		$Cx$ & force coefficient in the \textit{x} direction \\
		$Cy$ & force coefficient in the \textit{y} direction \\
		c   & chord \\
		d$t$ & time step \\
		$Fx$ & $X$ component of the resultant pressure force acting on the vehicle \\
		$Fy$ & $Y$ component of the resultant pressure force acting on the vehicle \\
		$f, g$   & generic functions \\
		$h$  & height \\
		$i$  & time index during navigation \\
		$j$  & waypoint index \\
		$K$  & trailing-edge (TE) nondimensional angular deflection rate\\
		$\Theta$ & boundary-layer momentum thickness\\
		$\rho$ & density\\
		\multicolumn{2}{@{}l}{Subscripts}\\
		cg & center of gravity\\
		$G$ & generator body\\
		iso	& waypoint index
\end{longtable*}}

